Prompt-Aware Scheduling for Efficient Text-to-Image Inferencing System

Traditional ML models utilize controlled approximations during high loads, employing faster, but less accurate models in a process called accuracy scaling. However, this method is less effective for generative text-to-image models due to their sensitivity to input prompts and performance degradation caused by large model loading overheads. This work introduces a novel text-to-image inference system that optimally matches prompts across multiple instances of the same model operating at various approximation levels to deliver high-quality images under high loads and fixed budgets.

==> tex/discussion.tex <==

\subsection{Other analysis}

\textbf{Quality-per-\$:} 
As we compare different type of systems that can introduce different kinds of approximations to increase the throughput under fixed cluster size or can use horizontal-scaling to serve high-loads, we introduce a new metric called \textit{quality-per-\$} to objectively compare the cost-effectiveness of different text-to-image serving systems.

\begin{table}[H]
    \centering
    \small
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Workload}} & \multicolumn{7}{c|}{\textbf{Quality-per-\$ }} \\ \cline{2-8}
         & {CHA} & {CHT} & {NRV} & {SOM} & {PRU} & {PAC} & {ACS} \\ \hline
        {Twitter} & 0.79 & 0.91 & 0.82 & 0.81 & 0.81 & 0.89 & 1.0 \\ \hline
        {Bursty} & 0.57 & 0.83 & 0.64 & 0.72 & 0.84 & 0.90 & 1.0 \\ \hline
        {SysX} & 0.62 & 0.92 & 0.86 & 0.83 & 0.76 & 0.85 & 1.0 \\ \hline
    \end{tabular}
    \caption{Quality-per-\$ for Clipper-HA(CHA), Clipper-HT(CHT), \NIRVANA(NRV), Sommelier(SOM), Proteus(PRU), PAC, and relative to \sys(ACS), for different workloads.}
    \label{tab:quality_per_dollar}
\end{table}


Table ~\ref{tab:quality_per_dollar} contains relative Quality-per-\$ for different methods across different workloads. From the table, it is clear that relatively \sys offer the best Quality-per-\$ for the text-to-image generation task.


\label{sec:otheranalysis}
We now present detailed runtime analysis of \sys.


\begin{figure}[H]
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholders/eval_degradaion_agnostic.pdf}
        \caption{Degradation with \sys's Prompt-Aware routing is (2-5\%) lower as compared to Prompt-Agnostic Routing.}
        \label{fig:degradation}
    \end{minipage}
    % \hfill
    \begin{minipage}{0.45\linewidth}

    \centering
        \includegraphics[width=\linewidth]{figures/placeholders/scale_solver.pdf}
        \caption{MILP solver scales well with the number of nodes in cluster with solving time in order of $ms$ for tens of nodes.}
        \label{fig:scale}
    \end{minipage}
\end{figure}



\textit{\textbf{High load-Low load analysis}}: We analyze the fraction of \sys runtime spent in low-vs-high load regimes (\S\ref{}) in Fig.~\ref{fig:load time}. 
For the twitter trace, the runtime is dominated with low-load model, whereas for the other two workloads, both high-load and low-load have significant runtime. This also explains the performance of \sys vs baselines. 
As seen in Fig.\ref{fig:high_low}, for Bursty and SysX, \sys shows a higher average quality drop with higher gains in average throughput and lower SLO violations ratio compared to the other baselines in the other two workloads as compared to Twitter trace. This is also true in \textit{Quality-per-\$} stats shown in Table \ref{tab:quality_per_dollar}. The primary reason being, at low-load mode, the model running is all large as the load is low. Also, the greedy packing only kicks in only at high-load mode. Since twitter trace has mostly low-load mode running, the benefit of these two components are seen less pronounced on average as compared to the other two workloads. However, in Fig. \ref{fig:performance_trace}, the time series clearly shows how \sys shows better throughput and generation quality  at high load conditions.  



\begin{figure}[H]
        \centering
        \includegraphics[width=\linewidth]{figures/placeholders/counts_batch.pdf}
        \caption{Batch size and count variants running at different workloads. Effective batch size changes from 1 to 2-4 as load increases. Slower K=0 variants are active at low loads. It switches to a mix of variants at higher loads, and finally only faster K = 25 variants running at peak loads.}
        \label{fig:counts_batch}
\end{figure}

\textit{\textbf{Variant runtime and switching analysis}}: For the runtime of \sys, we also analyze in Fig.~\ref{fig:counts_batch}, what all variants are running at few load times and the effective batch count active during those runtime for the Twitter trace workload. As seen in the plots, we see that a batch size of 1 is active for low workloads, and \sys switches to using batch size of 2 to 4 to maximize throughput and serve queries with a speedup inference using 
\textit{Flexi-batching}. The K variants active change as load changes, with all $K=0$ models running at low loads, a mix of models running at moderate loads, and all $K=25$ models running at high loads. Now, as few other baselines like Proteus and PAC also share the same MILP for model selection, frequent changes in model selection happens for them as well. However, since they use variants and not \AC models, they have high loading overheads. On average, these approaches tend to switch some variant around 27\%, 6\% and 42\% times of all decisions made by solver (running every minute), which leads to huge loading overheads, results in high SO violations and lower system throughput (around 15-20\% worse) overall. 


\begin{figure}[H]
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{figures/placeholders/load_fractions.pdf}
        \caption{\sys operates in low-load mode for 80\% of run time in Twitter trace. However, high-load is active for around 50\% of the runtime for others.}
        \label{fig:high_low}
    \end{minipage}
    \hspace{0.2em}
    \begin{minipage}{0.55\linewidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figures/placeholders/pred_error_hk.pdf}
        \caption{Error in predicting $\mathcal{H_k}$ looking at past K's for different window sizes gets lower and saturates around 1000.}
        \label{fig:pred_error}
    \end{minipage}
\end{figure}

\textit{\textbf{Scalability}}: The solver should run efficiently at a regular interval or when the load or distribution of $h_k$ changes suddenly. We test the scalability of the MILP solver for different GPU count in Fig. \ref{fig:scale}. For a cluster with tens of GPUs, the solver time is within $100$\textit{ms}, making it easy to scale. 

\textit{\textbf{$\mathcal{H}_k$ prediction}}: For an $\mathcal{F}_k$ provided by the MILP solver, the ODA then relies on prediction of $\mathcal{H}_k$ from Affinity Decider to decide the \textit{SG}. We show in the L2 prediction error for $\mathcal{H}_k$ Fig.~\ref{fig:pred_error} for different past window sizes of $K'$ logs. For the chosen value of 1000, it saturated at low error at around $0.01$. 



\subsection{Discussions}

\saold{
\label{sec:discussion}

\textbf{Genaralizability to other systems beyond diffusion/text-to-image/approximate caching.}

\textbf{Same base model different K.}
We do not switch models. Our inference works on throughput-accuracy by just varying K. So, there is no loading/unloading involved.

\textbf{Heterogeneous devices.}
The idea of model-less inferencing using caching can be easily extended to support heterogeneous device setting, with different GPU types. Specifically, when we use caching, the base model remains same, and hence run-time of different K on different GPU distances is just K dependent, if we profile the base model run time, making it trivial to extend. Even placement is trivial, as it is same base model.


\textbf{Reproducibility.}
Same input might give different outputs depending on the load + cache state.
Not a big deal for text-image may be which inherently are notg designed for repordicibility. + Other points.

\textbf{Change in prompt characteristics.}
If the characteristics of the prompts suddenly change due to some external factors, \sys will find less similar items in the cache and will automatically move towards lower $K$ or even for more dissimilar prompts the \matchpredictor will kick in and redirect the prompts to vanilla diffusion process. While this will reduce compute savings, \textit{by design} \sys will not let the image quality degrade in case of a sudden change in prompt characteristics.    

\textbf{ML optimizations.} 
Several techniques are used to reduce the compute footprint and latency of models such as use of lower precision~\cite{}, distillations~\cite{}, pruning~\cite{}, batched-inference optimizations~\cite{}. 
\sys is complementary to such techniques as it can be used on top of those optimized model as well to reduce redundant computation using approximate-caching.
However, a new family of generative models emerge that does not require such large number of iterative steps, then \sys's applicability will become limited. But since as of today, \dms with 50 or more denoising steps produce the best and production quality images, \sys provides an attractive proposition for compute reduction.     

}

\textbf{Limitations:} One of the main limitations of \sys is its usage of \AC that is applicable to models such as \dms that iteratively denoise/refine an image. However, since almost all of the production~\cite{firefly, dall-e, StableDi40:online}, as well as recent state of the papers~\cite{deci_diffusion, weng2021diffusion, croitoru2023diffusion, dhariwal2021diffusion, li2023qdiffusion}, on text-to-image models use \dms of various flavors, we argue that this model family us going to stay in near future. Moreover, the core algorithm of \sys that assigns prompts to particular model instance running at different approximation-latency configuration can also be seamlessly applied to a setup with multiple models that do not use iterative denoising.
The second drawback is that, micromanaging prompts has its limits. In the extreme case, if the load to the system increases so much that all the instance of the model has to run with maximum approximation levels, then the prompt assignment heuristic in \sys would not have any room to increase the quality. We argue that in that case, accuracy-scaling would not sustain and the system has to use traditional horizontal-scaling to sustain throughput under such extreme load. 

\begin{figure}[th]
    \begin{minipage}{0.9\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/placeholders/max_drop.pdf}
        \caption{\sys shows the lowest maximum drop in quality compared to all the other scaling methods (\textbf{20-30\%} lower than that of Sommelier and Proteus) across all the workloads.}
        % \sm{Quote, not needed in main paper}
        \label{fig:max_drop}
    \end{minipage}
\end{figure}


